Decoding Communications with Partial Information

Machine language acquisition is often presented as a problem of imitation learning: there exists a community of language users from which a learner observes speech acts and attempts to decode the mappings between utterances and situations. However, an interesting consideration that is typically unaddressed is partial observability, i.e. the learner is assumed to see all relevant information. This paper explores relaxing this assumption, thereby posing a more challenging setting where such information needs to be inferred from knowledge of the environment, the actions taken, and messages sent. We see several motivating examples of this problem, demonstrate how they can be solved in a toy setting, and formally explore challenges that arise in more general settings. A learning-based algorithm is then presented to perform the decoding of private information to facilitate language acquisition.

==> preamble.tex <==
% ************************* Algorithms and Pseudocode **************************

%\usepackage{algpseudocode}
% \usepackage{algorithm}
% \usepackage{algorithmic}
\usepackage[ruled]{algorithm2e}
  
% ********************Captions and Hyperreferencing / URL **********************

% Captions: This makes captions of figures use a boldfaced small font.
%\RequirePackage[small,bf]{caption}

\RequirePackage[labelsep=space,tableposition=top]{caption}
\renewcommand{\figurename}{Fig.} %to support older versions of captions.sty


% *************************** Graphics and figures *****************************

%\usepackage{rotating}
\usepackage{wrapfig}

% Uncomment the following two lines to force Latex to place the figure.
% Use [H] when including graphics. Note 'H' instead of 'h'
%\usepackage{float}
%\restylefloat{figure}

% Subcaption package is also available in the sty folder you can use that by
% uncommenting the following line
% This is for people stuck with older versions of texlive
%\usepackage{sty/caption/subcaption}
\usepackage{subcaption}

% ********************************** Tables ************************************
\usepackage{booktabs} % For professional looking tables
\usepackage{multirow}

%\usepackage{multicol}
%\usepackage{longtable}
%\usepackage{tabularx}

\usepackage{siunitx} % use this package module for SI units

\usepackage{enumitem}

\usepackage{graphicx}
\usepackage{float}
\usepackage{tikz}
% \usepackage[utf8]{inputenc}
% \usepackage{lmodern}
% \usepackage[T1]{fontenc} aaai forbidden
% \usepackage{xparse}

\usepackage{dsfont}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{mathtools}

\usepackage{bm}

\usepackage{diagbox}

\newcommand{\citepos}[1]{\citeauthor{#1}'s (\citeyear{#1})}

\usepackage{totcount}

\newtotcounter{citnum} %From the package documentation
\def\oldbibitem{} \let\oldbibitem=\bibitem
\def\bibitem{\stepcounter{citnum}\oldbibitem}

% \newcommand{\chapabstract}[1]{
%     \begin{quote}
%         \singlespacing\small
%         \rule{\linewidth}{1pt}
%         \vskip.5mm
%         \textbf{Chapter Abstract.} #1
%         % \vskip-4mm
%         \rule{\linewidth}{1pt}
%     \end{quote}%
% }

% \newtheoremstyle{mystyle}%                % Name
%   {}%                                     % Space above
%   {}%                                     % Space below
%   {\itshape}%                                     % Body font
%   {}%                                     % Indent amount
%   {\bfseries}%                            % Theorem head font
%   {.}%                                    % Punctuation after theorem head
%   { }%                                    % Space after theorem head, ' ', or \newline
%   {}%                                     % Theorem head spec (can be left empty, meaning `normal')

% \theoremstyle{plain}
% \theoremstyle{mystyle}

\newenvironment{proofsketch}{%
  \renewcommand{\proofname}{Proof sketch}\proof}{\endproof}

\newtheorem{problem}{Problem}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[section]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}{Example}
\newtheorem*{excont}{Example \textnormal{\continuation}}
\newcommand{\continuation}{??}
\newenvironment{continueexample}[1]
{\renewcommand{\continuation}{\ref{#1}}\excont[continued]}
{\endexcont}
\usepackage[utf8]{inputenc}

% \numberwithin{problem}{chapter}
% \numberwithin{example}{chapter}
% % \numberwithin{definition}{chapter}
% % \numberwithin{lemma}{chapter}
% \numberwithin{theorem}{chapter}

\usepackage{lipsum}


% \input{Preamble/macros}

% \pdfminorversion=6
\usepackage{nameref}

% \usepackage{minted}
% \usemintedstyle{vs}

% % inline python command
% \newcommand{\pyi}[1]{\mintinline{Python}{#1}}


\newcommand{\envstratequiv}[0]{{\mathbin{\stackrel{e}{\equiv}}\,}}
\newcommand{\commstratequiv}[0]{{\mathbin{\stackrel{c}{\equiv}}\,}}

\usepackage{amssymb}


\usepackage[toc,acronym]{glossaries}
% \usepackage[toc,acronym]{glossaries-extra}

% \usepackage[postdot]{glossaries-extra}
% \usepackage[xindy]{glossaries-extra}

\preto\chapter{\glsresetall}

\makeglossaries{}

% \GlsXtrEnablePreLocationTag{(page }{(pages }
% \renewcommand{\GlsXtrFormatLocationList}[1]{#1)}

% \GlsXtrEnablePreLocationTag{Page: }{Pages: }

\newacronym[plural=MDPs,firstplural=Markov Decision Processes (MDPs)]{mdp}{MDP}{Markov Decision Process}

\newacronym[plural=POMDPs,firstplural=Partially Observable Markov Decision Processes (POMDPs)]{pomdp}{POMDP}{Partially Observable Markov Decision Process}

\newacronym[plural=Dec-POMDPs]{decpomdp}{Dec-POMDP}{Decentralised Partially-Observable Markov Decision Process}

\newacronym[plural=Comm-Dec-POMDPs,firstplural=Decentralised Partially Observable Markov Decision Processes with Communications (Comm-Dec-POMDPs)]{comm-decpomdp}{Comm-Dec-POMDP}{Decentralised Partially-Observable Markov Decision Process with Communication}

% \newacronym[plural=Dec-POMDPs,firstplural=Decentralised Partially Observable Markov Decision Processes (POMDPs)]{pomdp}{Dec-POMDP}{Decentralised Partially Observable Markov Decision Process}

\newacronym[plural=GRNs]{grn}{GRN}{Gene Regulatory Network}

\newacronym[plural=GAs]{ga}{GA}{Genetic Algorithm}

\newacronym{ea}{EA}{Evolutionary Algorithm}

\newacronym{zsc}{ZSC}{Zero-Shot Coordination}

\newacronym{ai}{AI}{Artificial Intelligence}

\newacronym{alife}{ALife}{Artificial Life}

\newacronym{il}{IL}{Imitation Learning}

\newacronym{bc}{BC}{Behaviour Cloning}

\newacronym{ml}{ML}{Machine Learning}

\newacronym{llm}{LLM}{Large Language Model}

\newacronym{dl}{DL}{Deep Learning}

\newacronym{ood}{OoD}{Out-of-Distribution}

\newacronym{ind}{InD}{In-Distribution}

\newacronym{nlp}{NLP}{Natural Language Processing}

\newacronym{aht}{AHT}{Ad Hoc Teamwork}

\newacronym[plural=DNNs]{dnn}{DNN}{Deep Neural Network}

\newacronym[plural=ANNs]{ann}{ANN}{Artificial Neural Network}

\newacronym[plural=RNNs]{rnn}{RNN}{Recurrent Neural Network}

\newacronym[plural=CNNs]{cnn}{CNN}{Convolutional Neural Network}

\newacronym{dial}{DIAL}{Differentiable Inter-Agent Learning}

\newacronym{dru}{DRU}{Discretise/Regularise Unit}

\newacronym{dqn}{DQN}{Deep Q-Network}

\newacronym{td}{TD}{Temporal Difference}

\newacronym{pg}{PG}{Policy Gradient}

\newacronym{twean}{TWEANN}{Topology and Weight Evolving Artificial Neural Networks}

\newacronym{neat}{NEAT}{NeuroEvolution of Augmenting Topologies}

\newacronym{rl}{RL}{Reinforcement Learning}

\newacronym{drl}{DRL}{Deep Reinforcement Learning}

\newacronym{rlhf}{RLHF}{Reinforcement Learning from Human Feedback}

\newacronym{irl}{IRL}{Inverse Reinforcement Learning}

\newacronym{ctde}{CTDE}{Centralised Training with Decentralised Execution}

\newacronym{marl}{MARL}{Multi-Agent Reinforcement Learning}

\newacronym{dmarl}{DMARL}{Deep Multi-Agent Reinforcement Learning}

\newacronym{iql}{IQL}{Independent Q-Learning}

\newacronym{qmix}{QMIX}{Q-Mix}

\newacronym{vdn}{VDN}{Value-Decomposition Network}

\newacronym{ppo}{PPO}{Proximal Policy Optimisation}

\newacronym{mappo}{MAPPO}{Multi-Agent Proximal Policy Optimisation}

\newacronym{maddpg}{MADDPG}{Multi-Agent Deep Deterministic Policy Gradient}

\newacronym{ec}{EC}{Emergent Communication}

\newacronym{ectl}{ECTL}{Emergent Communication pretraining and Translation Learning}

\newacronym{clap}{CLAP}{Cooperative Language Acquisition Problem}

\newacronym{clap-replace}{CLAP-Replace}{CLAP Replacement Task}

\newacronym{poclap}{POCLAP}{Partially-Observable Cooperative Language Acquisition Problem}

\newacronym{poclap-replace}{POCLAP-Replace}{POCLAP Replacement Task}

\newcommand{\Description}[1]{}

